Towards Lifelong Federated Learning in Autonomous Mobile Robots with Continuous Sim-to-Real Transfer

The role of deep learning (DL) in robotics has significantly deepened over the last decade. Intelligent robotic systems today are highly connected systems that rely on DL for a variety of perception, control, and other tasks. At the same time, autonomous robots are being increasingly deployed as part of fleets, with collaboration among robots becoming a more relevant factor. From the perspective of collaborative learning, federated learning (FL) enables continuous training of models in a distributed, privacy-preserving way. This paper focuses on vision-based obstacle avoidance for mobile robot navigation. On this basis, we explore the potential of FL for distributed systems of mobile robots enabling continuous learning via the engagement of robots in both simulated and real-world scenarios. We extend previous works by studying the performance of different image classifiers for FL, compared to centralized, cloud-based learning with a priori aggregated data. We also introduce an approach to continuous learning from mobile robots with extended sensor suites able to provide automatically labeled data while they are completing other tasks. We show that higher accuracies can be achieved by training the models in both simulation and reality, enabling continuous updates to deployed models.

==> algs/pos_gd.tex <==


\begin{algorithm}[t]
    %
    %
    %
    \footnotesize
	\caption{\footnotesize Ground truth extraction}
	\label{alg:tracking}
	\KwIn{\\
	    \begin{tabular}{ll}
	        3D lidar point cloud:             & $\mathcal{P}$ \\
	        Last known MAV state:              & $ \textbf{p}^{k-1}_{MAV}, {\dot{\textbf{p}}_{MAV}}^{k-1}$ \\[+0.4em]
	    \end{tabular}
	}
	\KwOut{\\
	    \begin{tabular}{ll}
	        MAV state:      & \{${\textbf{p}^{k}_{MAV}}, \:\dot{\textbf{p}}^{k}_{MAV}\}$ \\[+0.2em] 
	    \end{tabular}
	}  
	%\BlankLine
	%
	\SetKwFunction{FSub}{$object\_extraction\left(\mathcal{P}, \:{\textbf{p}^{k-1}_{MAV}}, \:\dot{\textbf{p}}^{k-1}_{MAV}\right)$}
    \SetKwProg{Fn}{Function}{:}{}
    % Position estimation based on current PointCloud and last position and speed
    \BlankLine
%     \Fn{\FSub}
%     {
%             \vspace{.3em}
            
%             \KwRet ${\textbf{p}^{k}_{MAV}};$
%     }
% 	\BlankLine
    %
% 	$Adaptive\;Integrate\;Rate: I_{rate}$ \\
    % Calculate with high frequency, get the pose(high accuracy, but not robust)  
    % Coarse first, then fine grained estimate
    % \tcp{Coarse but persistent tracking}
    % \While{new $\mathcal{P}_{k}(I^{k}_{MF})$}{
    %     ${\textbf{p}^{k'}_{MAV}} =  object\_extraction(\mathcal{P}_{k}(I^{k}_{MF}), I^{k}_{MF}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
    %     % $Evaluate \; Estimation({\textbf{p}^{k-1}_{MAV}}, {\textbf{p}^{k}_{MAV}} )$ \\
    %     % $Update({\textbf{p}}^{k}, I_{rate} )$ \\
    % }
    % \tcp{Fine-grained estimation}
    \While{new $\mathcal{P}_{k}$}{
        \begin{tabular}{ll}
                Generate KD Tree:       & $kdtree \leftarrow \mathcal{P};$ \\
                MAV pos estimation:     & $\hat{\textbf{p}}_{\tiny MAV}^{k} \leftarrow \textbf{p}^{k-1}_{MAV} + \frac{\dot{\textbf{p}}_{MAV}^{k-1}}{I};$ \\[+0.4em]
                MAV points:             & $\mathcal{P}^{k}_{MAV} = KNN(kdtree, \: \hat{\textbf{p}}_{MAV}^{k});$ \\[+0.4em]
                MAV state estimation:   & ${\textbf{p}^{k}_{MAV}} = \frac{1}{\lvert\mathcal{P}^{k}_{MAV}\rvert}\sum_{p\in\mathcal{P}^{k}_{MAV}} p;$ \\
        \end{tabular}
        % ${\textbf{p}^{k''}_{MAV}} =  object\_extraction(\mathcal{P}_{k}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
        % ${\textbf{p}^{k}_{MAV}}, \: {\dot{\textbf{p}}^{k}_{MAV}} \leftarrow estimate\left(\textbf{p}^{k'}_{MAV}, \:\textbf{p}^{k''}_{MAV}\right)$\;
    }
    % $\{I^{k}_{HF}, I^{k}_{MF}\} \leftarrow adjust\_integration\_freqs\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$ \\[+0.4em]
    % $\dot{\textbf{q}}^{k}_{UGV} \leftarrow keep\_within\_FoV\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$
    
 
\end{algorithm}

==> tex/data_distribution_table.tex <==

% \begin{table}
%     \centering
%     \caption{Distribution of Data from Three Simulated Environments and Three Real-World Rooms}
%     \label{tab:data_distribution}
%     \footnotesize
%     \begin{tabular}{@{}lcccccc@{}}
%     \toprule
%     \multirow{2}{*}{}              & \multicolumn{2}{*}{\textbf{Hospital / Room 1}}       & \multicolumn{2}{*}{\textbf{Office / Room 2}}         & \multicolumn{2}{*}{\textbf{Warehouse / Room 3}}                      \\
%     & \multicolumn{1}{*}{\textbf{\scriptsize{BLOCKED}}} & \textbf{free} & \multicolumn{1}{*}{\textbf{blocked}} & \textbf{free} & \multicolumn{1}{*}{\textbf{blocked}} & \textbf{free}                       \\
%     \midrule
%     \textbf{Sim} & \multicolumn{1}{*}{44\%}             & 56\%          & \multicolumn{1}{*}{64\%}             & 46\%          & \multicolumn{1}{*}{60\%}             & 40\%                        \\
%     \multirow{2}{*}{\textbf{Real}} & \multicolumn{1}{*}{40\%}             & 60\%          & \multicolumn{1}{*}{50\%}             & 50\%          & \multicolumn{1}{*}{50\%}             & 50\%                        \\
%     & \multicolumn{2}{*}{11\%}                             & \multicolumn{2}{*}{44\%}                             & \multicolumn{2}{*}{45\%}                              \\ 
%   \bottomrule
%     \end{tabular}
% \end{table}


% hospital: 145, 181
%           blocked, free
% warehouse: 351, 297
%           blocked, free
% office:  196, 130
% 

==> tex/fuse_combinations.tex <==
\begin{table}[t]
    \centering
    \caption{\footnotesize Fused Model Combination Acronyms}
    \label{tab:fuse_combination}
    \scriptsize
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        \textbf{Combinations} & \textbf{M0\&M1} & \textbf{M0\&M2} & \textbf{M1\&M2} & \textbf{M0\&M1\&M2} \\ 
        \midrule
        \textbf{Acronyms}     & M01                & M02                & M12                & M012                      \\ 
        \bottomrule
    \end{tabular}
\end{table}
